Enhanced Fairness Testing via Generating Effective Initial Individual Discriminatory Instances

Fairness testing aims at mitigating unintended discrimination in the decision-making process of data-driven AI systems. Individual discrimination may occur when an AI model makes different decisions for two distinct individuals who are distinguishable solely according to protected attributes, such as age and race. Such instances reveal biased AI behaviour, and are called Individual Discriminatory Instances (IDIs). In this paper, we propose an approach for the selection of the initial seeds to generate IDIs for fairness testing. Previous studies mainly used random initial seeds to this end. However this phase is crucial, as these seeds are the basis of the follow-up IDIs generation. We dubbed our proposed seed selection approach I&D. It generates a large number of initial IDIs exhibiting a great diversity, aiming at improving the overall performance of fairness testing. Our empirical study reveal that I&D is able to produce a larger number of IDIs with respect to four state-of-the-art seed generation approaches, generating 1.68X more IDIs on average. Moreover, we compare the use of I&D to train machine learning models and find that using I&D reduces the number of remaining IDIs by 29% when compared to the state-of-the-art, thus indicating that I&D is effective for improving model fairness

==> acknowledgements.tex <==
Junjie Chen 

Chuan Luo 

data links 
https://archive.ics.uci.edu/ml/datasets/adult
https://archive.ics.uci.edu/ml/datasets/bank+marketing
https://github.com/propublica/compas-analysis

==> coverletter.tex <==
\hfill{\today}

ACM Transactions on Software Engineering and Methodology


\bigskip

Dear Editors,

\bigskip

We are writing to submit our manuscript ``Enhanced Fairness Testing via Generating Effective Initial Individual Discriminatory Instances'' to the \emph{ACM Transactions on Software Engineering and Methodology}, 	Continuous Special Section: AI and SE.

Software systems utilize Artificial Intelligence (AI in various application areas, often times when dealing with sensitive information such as gender or race of individuals.
To avoid unintended bias in the decision-making process of data-driven AI systems, a growing attention is paid to fairness testing.
In particular, fairness testing is applied with regards to individual fairness (i.e., two individuals that are identical except for sensitive attributes are treated differently).
For this purpose, fairness testing approaches set out to detect Individual Discriminatory Instances (IDIs), to gauge the bias of machine learning models.
The IDIs detection phase follows three stages: 1) Initial seed selection; 2) Local Generation; 3) Global generation.
While existing approach focus on the later two, we propose a novel approach, named \textit{I\&D}, to improve the initial seed selection stage,
which can be used to extend existing approaches.

Specifically, this paper makes the following contributions:
\begin{itemize}
    \item We perform the first study dedicated to the selection of initial IDIs for improving fairness testing.
    \item We design a method called \name to for creating a diverse set of IDIs.
    \item We conduct a comprehensive empirical assessment of \name based on three public datasets and four existing IDI generation approaches.
\end{itemize}

\noindent
We believe that this paper lies in the scope of TOSEM, and especially its 	Continuous Special Section on AI and SE, as we investigate software testing techniques with regards to the non-functional property of \textit{fairness} for machine learning software. Moreover, this paper presents novel work and has not been presented or published before.

Thanks for your upcoming efforts on reviewing our work. We look forward to hearing from you.
 
\bigskip
Best regards,

The authors 

Minghua Ma 

Zhao Tian

Max Hort 

Federica Sarro 

Hongyu Zhang 

Qingwei Lin 

Dongmei Zhang









% We suggest the following Associate Editors and reviewers for our submission.

% Associate Editors:
% \begin{itemize}
%     \item Burak Turhan
%     \item Baishakhi Ray
%     \item Sam Malek
% \end{itemize}

% Reviewers:
% \begin{itemize}
%     \item Sudipta Chattopadhyay, Singapore University of Technology and Design (sudipta\_chattopadhyay@sutd.edu.sg)
%     \item Sun Jun, Singapore Management University (junsun@smu.edu.sg)
% \end{itemize}

% We would also like to note the following conflicts of interest:
% %Federica Sarro is Associate Editor for the TOSEM Journal.

% \point{All of the TOSEM Associate Editors an author on the submission may have a conflict with} 

% Paolo Tonella

% Shin Yoo

% \point{All of the TOSEM Distinguished Reviewers an author on the submission may have a conflict with} 
% %https://dl.acm.org/journal/tosem/distinguished-reviewers-board

% Carmine Gravino

% \point{We list below all collaborators and their affiliations (for all authors on the paper) in the past 5 years}

% Tsinghua University 

% Tianjin University 

% Microsoft

% University College London 

% The University of Newcastle

% META (formerly Facebook)

% \point{The name of the universities and industry sites the author's graduated from/are affiliated with and the name of the author's adviser}

% Minghua Ma graduated from Tsinghua University. His adviser is Professor Dan Pei. He is currently at Microsoft Research Lab Asia.

% Federica Sarro graduated from University of Salerno, adviser Professor Filomena Ferrucci. She is currently at University College London.


==> rebuttal.tex <==
Thanks for your valuable comments and supportive feedback about our work. We respond below to each of the questions asked. We hope this can provide you with the clarifications required to support the acceptance of our work, as we believe we can carefully address in the camera-ready version all points raised.

\textbf{Review \#35A}

\textbf{Q1. I\&D requires the dataset} 
Yes, I\&D and clustering-based approach require the dataset. While random seed initialization does not operate directly on the dataset, information about the input space is still required (i.e., what are possible values for each attribute). 

\textbf{Q2. Why is training a chiral model and computing SHAP values the best way to address this problem?}
The benefit of using a chiral model in combination with SHAP values is that one is not only able to detect IDIs (as it could have been done with a random modification of protected attributes) but can also ensure that they possess a high diversity. This is relevant for the performance of fairness testing techniques as investigated in Section 4.3. We will further clarify this in the paper. Feeding the output of one technique (e.g., SG) as the initial seed selection to another technique, or to itself, could be an interesting extension of this study. While this could allow for additional IDIs found by local search, it would require a higher computational overhead than the approach proposed herein. We will include these future works in the paper.


\textbf{Review \#35B}

\textbf{Q1. Overhead of training Chiral Model}
Table 3 shows that the overhead of training the Chiral Model is less than three seconds. Although the model we utilized in the experiment is relatively simple and its running time negligible, we observe that the overhead due to the training phase might be further reduced by training the chiral model sharing parameters with the original model. We will include this observation in the paper.

\textbf{Q2. Design choices}
The original model and chiral model are both trained on data taken from the original dataset (with mutation of protected attributes for the chiral model). For more details on design choices, please refer to Review\#35A-Q2.


\textbf{Review \#35C}

\textbf{Q1. How realistic are the generated IDIs?}
Individual Discriminatory Instances (IDIs) are defined and widely-adopted in previous studies [3,35,41,42]. The question of correlated attributes is concerned with group fairness rather than individual fairness definitions.

\textbf{Q2. P-values} 
Our aim is to assess to what extent I\&D is effective when combined with different approaches. Therefore, we used the Wilcoxon test to test for the following null hypothesis \textit{The use of I\&D does not improve the performance of AEQ, SG, ADF and EIDIG.} and we compared the distribution of results obtained with [I\&D+AEQ, I\&D+SG, I\&D+ADF and I\&D+AEQ+EIDIG] vs. the distribution of the results obtained with [AEQ, SG, ADF and EIDIG] over all datasets and 10 runs. This resulted in the p-value reported in the paper.

\textbf{Q3. 60-40 split}
For this design choice we followed previous work which also used a train-test split (e.g., [41]). Similar to cross-validation, we train classifiers 10 times and average performance results. We will further clarify this point in the paper, and explain that other types of cross-validation could be used in future work. 

\textbf{Q4. Fairness metrics}
Disparate Impact, Statistical Party and Demographic Parity are \textit{group fairness metrics} that have been used for evaluating the performance of bias mitigation methods  for classifiers.
Whereas, fairness testing is concerned with individual discrimination and therefore utilizes a different set of metrics (\textit{individual fairness metrics}). Since our work addresses fairness testing (and not bias mitigation methods), we utilize individual fairness metrics.

\textbf{Q5. Relevance to SE}
Software engineers evaluate software quality mainly through software testing.
Fairness is a crucial quality attribute of ML-enabled software. Our work aims at enhancing previous methods proposed to automatically generate test suites that measure discrimination (i.e., improve fairness). 
We understand that fairness testing has only been recently tackled in SE, but it is long overdue, as pointed out in Brun and Meliou’s work [9], who later on won the IEEE CS TCSE New Directions Award for setting a new direction in software engineering research by defining the area of software fairness testing. In their seminal paper at FSE'17, “Fairness Testing: Testing Software for Discrimination,” which won an ACM SIGSOFT Distinguished Paper Award, Galhotra et al. [17] presented the first concrete technique for automated fairness test suite generation. With the use of fairness testing, developers can ensure and validate the fairness of ML-enabled software. Since then, fairness testing work has appeared in SE venues such as FSE [3], ASE [35], ISSTA [41] and ICSE [42]. We provide more details in Section 5.

\textbf{Q6. Percentage}
The percentage varies across datasets and IDI generation limit, ranging from 1.3\% to 4.9\%. 

\textbf{Additional Clarifications}

\textbf{Review \#35A} 

\textbf{No comparison with baselines}: We compare with two baselines, i.e. random sampling[35] and clustering based sampling[3,41,42] (see Section 4.2). 

\textbf{Review \#35B}

\textbf{Experimental choices about Aequitas} We compare with fully-directed Aequitas.

\textbf{How does the approach work if the datasets are more complex?}
Our approach is only applied on tabular data, similar to the existing fairness testing studies [3,35,41,42]. It can be transferred to other domains, including image or text, if there is access to a binary protected attribute. We will discuss this as possible future work.

\textbf{Review \#35C}

\textbf{Datasets} 
As explained in the paper (line 1080), we did not include the German dataset in the current version due to its small size, and thus the higher chance of overfitting. However, we can also include these results in the camera-ready of our paper if the reviewers believe it is important/interesting.

\textbf{Requires retraining}
Retraining is a standard practice in fairness testing to evaluate the quality of generated IDIs.

\textbf{Non-determinism and complex model}
Due to the non-determinism of Neural Networks, we can not ensure that retraining always leads to improvements, however this does not imply that I\&D is not applicable to complex models. Independent of the model complexity, a chiral model can be trained as long as a binary protected attribute is present.
To alleviate the risk of non-determinism and to show the ability of I\&D to improve large models, such as Neural Networks, we report the performance over 10 repetitions. We will clarify these aspect in the paper.

\textbf{Writing}
We will carefully proof-read the paper and improve the presentation.
